Minimizing the Age of Information through Queues

In this paper, we investigate scheduling policies that minimize the age of information in single-hop queueing systems. We propose a Last-Generated, First-Serve (LGFS) scheduling policy, in which the packet with the earliest generation time is processed with the highest priority. If the service times are i.i.d. exponentially distributed, the preemptive LGFS policy is proven to be age-optimal in a stochastic ordering sense. If the service times are i.i.d. and satisfy a New-Better-than-Used (NBU) distributional property, the non-preemptive LGFS policy is shown to be within a constant gap from the optimum age performance. These age-optimality results are quite general: (i) They hold for arbitrary packet generation times and arrival times (including out-of-order packet arrivals), (ii) They hold for multi-server packet scheduling with the possibility of replicating a packet over multiple servers, (iii) They hold for minimizing not only the time-average age and mean peak age, but also for minimizing the age stochastic process and any non-decreasing functional of the age stochastic process. If the packet generation time is equal to packet arrival time, the LGFS policies reduce to the Last-Come, First-Serve (LCFS) policies. Hence, the age optimality results of LCFS-type policies are also established.

==> sections/Discussion.tex <==
\section{Discussion}\label{Disc}
In this section, we discuss our results and compare it with prior works. 
\subsection{Preemption vs. Non-Preemption}
In the conclusion of \cite[Appendix]{CostaCodreanuEphremides_TIT}, the authors claimed that "In  the  LCFS  system  with  preemption  we  expect  that,  for  very large  arrival  rates,  the  age  would  increase  without  bound,  as  no  packet  finishes  service''. This claim is correct when the packet service times are NBU. As we will see in Fig. \ref{avg_peak_age3}, the age of the preemptive LCFS policy grows to infinity at high traffic intensity for gamma distributed service times. However, preemption does not increase the age for exponential service times, because the remaining service times of a preempted packet has the same distribution with the service time of a new packet. In Theorem \ref{thm1}, we have proven that the preemptive LCFS policy is age-optimal for exponential service times and general system parameters. In Theorem 3(a) of \cite{RYatesTIT16}, Yates and Kaul showed that the average age of the preemptive LCFS policy is a decreasing function of the traffic intensity $\rho$ in M/M/1 queues as $\rho$ grows to infinite. 

%On one hand, this contradicts our results in Theorem \ref{thm1}, in which we showed that the LCFS system with preemption can, indeed, achieve age-optimality for all arrival rates among all causal policies when the service times are exponentially distributed and the update packets arrive in the order of their generation times. Moreover, the study in \cite{RYatesTIT16} showed that the preemptive LCFS policy achieves bounded average age for all arrival rates when the service times are exponentially distributed. However, for non-exponential service time, the age of the preemptive LCFS policy could blow up at high traffic intensity (as we will see in Fig. \ref{avg_peak_age3}). This is because the packet service times are no longer memoryless. Thus, high traffic intensity leads to increased preemption rate which, in turn, leads to no packet completes service. Hence, the inter-departure times increase causing the rise in the age. From this, we can deduce that the age performance of the prmp-LGFS-R policy depends essentially on the service time distribution.

In addition, the study in \cite{Gamma_dist} characterized the age for LCFS systems with and without preemption for  gamma distributed service times. In \cite[Numerical Results]{Gamma_dist}, the authors showed that the non-preemptive LCFS policy can achieve better average age performance than the preemptive LCFS policy. In this paper, we further show that the non-prmp-LGFS-R policy is within a small constant gap from the optimum expected average age for all NBU service time distributions, which include gamma distribution as one example.

%In addition, the study in \cite{Gamma_dist} characterized the age for LCFS systems with and without preemption when the service time is gamma distributed (gamma distribution belongs to the class of NBU distributions). In \cite[Numerical Results]{Gamma_dist}, the authors showed that the non-preemptive policy can achieve better average age than the preemptive one. In this paper, we showed that the non-prmp-LGFS-R policy can come close to age-optimal when the service time is NBU distributed. More specifically, the non-prmp-LGFS-R is within a small age gap from the optimum expected average age for NBU service times.

\subsection{Replication vs. Non-Replication}
The replication technique has gained significant attention in recent years to reduce the delay in queueing systems \cite{Chen_queue_coding,yin_data_retrieve,sun2016delay}. However, under some system settings, replications may worsen the delay performance. In particular, it was shown in \cite{sun2016delay} that replication policies are far from the optimum delay for NBU service time distributions. A simple explanation of this result is as follows: Let $X_1, X_2, \ldots, X_m$ be i.i.d. NBU random variables with mean $\mathbb{E}[X_l]=\mathbb{E}[X]<\infty$. From the properties of the NBU distributions, we can obtain \cite{joshi2017efficient}
\begin{equation}\label{NBUproperty_delay}
\mathbb{E}[\min_{l=1,\ldots,m}X_l]\geq \frac{\mathbb{E}[X]}{m}.
\end{equation}
Now, if $X_l$ represents the packet service time of server $l$, then the left-hand side of \eqref{NBUproperty_delay} represents the mean service time (the mean time spent by each server per packet) when each packet is replicated to all servers; and the right-hand side of \eqref{NBUproperty_delay} represents the mean service time when there is no replication. This gives insight why packet replication can worsen the delay performance when the service time is NBU. Somewhat to our surprise, we found in this paper that the non-prmp-LGFS-R policy is near-optimal in minimizing the age, even for NBU service time distributions. The intuition behind this result is that the age is affected by the freshness of the delivered packets irrelevant to the total number of delivered packets. In other words, to reduce the age, we need to deliver the freshest packet as soon as possible. Also, it is obvious that 
\begin{equation}
\mathbb{E}[\min_{l=1,\ldots,m}X_l]\leq\mathbb{E}[X].
\end{equation}
Thus, packet replication can help in this direction by exploiting the diversity provided by multiple servers. 
\subsection{New-Worse-than-Used service time distributions}
Another important class of distributions that are more general than exponential is New-Worse-than-Used (NWU) distributions. The definition of the NWU distributions is as follows: 
\begin{definition}  \textbf{New-Worse-than-Used distributions:} Consider a non-negative random variable $Z$ with CCDF $\bar{F}(z)=\mathbb{P}[Z>z]$. Then, $Z$ is \textbf{New-Worse-than-Used (NWU)} if for all $t,\tau\geq0$
\begin{equation}\label{NWU_Inequality}
\bar{F}(\tau +t)\geq \bar{F}(\tau)\bar{F}(t).
\end{equation} 
\end{definition}
Examples of NWU distributions include hyperexponential distribution, Weibull distribution with $c <1$, etc. A  random variable is both NBU and NWU if, and only if, it is exponential. We investigated whether age-optimality can be achieved when the service times are NWU. We figured out that no policy can achieve optimality when the service times are NWU. To clarify this claim, let us consider the following example.

 \begin{figure*}[!tbp]
 \centering
 \subfigure[Case 1: Preemption is allowed.]{
  \includegraphics[scale=0.3]{figure/NWU.eps}
   \label{1a}
   }
 \subfigure[Case 2: Preemption is not allowed.]{
  \includegraphics[scale=0.3]{figure/NWU2.eps}
   \label{2b}
   }
   \caption{Illustration of policies $\pi$ and $\pi'$ in the Example }
   \label{fig:samp_path_NBU}
\end{figure*}
\textbf{Example:}
\emph{Consider a single server queue with $U(0)=0$ for all policies. We first consider the case where preemption is allowed. Suppose that the policies $\pi$ and $\pi'$ start to process packet 1 at time 0, as shown in  Fig. \ref{1a}. Suppose that at time $\delta$, packet 2 with $s_2<s_1$ arrives at the system. Since $s_1>s_2$, an intuitive action is to keep processing the fresh packet (packet 1) and ignore the old packet (packet 2). We will show that this decision may not achieve lower age. Suppose that policy $\pi'$ preempts the processing of packet 1 and starts to serve packet 2 at time $\delta$ and completes the service of packet 2 at time $\gamma$, as shown in  Fig. \ref{1a}. Let $R_1$ represent the remaining service time to complete packet 1 at time $\delta$ under policy $\pi$. Suppose that the server has spent $\chi$ ($\chi\geq 0$) seconds on processing packet 1 by time $\delta$ in policy $\pi$. Define $X_1=\chi+R_1$ as the service time of packet 1 under policy $\pi$ and $X_2=\gamma-\delta$ as the service time of packet 2 under policy $\pi'$. Then, the CCDF of $R_1$ is given by
\begin{equation}\label{ex_NWU_1}
\mathbb{P}[R_1>t]=\mathbb{P}[(X_1-\chi)>t\vert X_1>\chi].
\end{equation}
Because the packet service times are NWU, we can obtain that for all $t, \chi\geq 0$
\begin{equation}\label{ex_NWU_2}
\mathbb{P}[(X_1-\chi)>t\vert X_1>\chi]=\mathbb{P}[(X_2-\chi_1)>t\vert X_2>\chi_1]\geq\mathbb{P}[X_2>t].
\end{equation}
Combining \eqref{ex_NWU_1} and \eqref{ex_NWU_2}, we get
\begin{equation}\label{ex_NWU_3}
R_1\geq_{\text{st}}X_2.
\end{equation}
This means that the completion time of packet 2 under policy $\pi'$ is stochastically smaller than the completion time of packet 1 under policy $\pi$, as shown in  Fig. \ref{1a}. Thus, policy $\pi'$ can obtain lower age at time $\gamma$ than policy $\pi$, i.e., we have
\begin{equation}
\Delta_\pi(\gamma)=\gamma\geq\gamma-s_2=\Delta_{\pi'}(\gamma).
\end{equation}}

\emph{Now, we proceed to the case where preemption is not allowed. We will show that a non-work-conserving policy can obtain lower age than the work-conserving one. Suppose that policy $\pi$ starts processing packet 1 at time 0; and policy $\pi'$ does idle the server until time $\delta$, then assigns packet 2 to the server, as shown in Fig. \ref{2b}. We assume here that $0=a_1<a_2\leq\delta$ and $s_2>s_1$. By the same argument as in the first case, we can show that the completion time of packet 2 under policy $\pi'$ is stochastically smaller than the completion time of packet 1 under policy $\pi$, as shown in Fig. \ref{2b}. This means that the non-work-conserving policy $\pi'$ can obtain a lower age than policy $\pi$.}

This example shows that age-optimality is extremely hard to be achieved within the policy space that includes all causal policies when the service times are NWU distributed. However, we showed in \cite{multihop_optimal} that optimality can be achieved for general service time in single server queues among all non-preemptive work-conserving policies.

==> sections/Numerical_results.tex <==
\section{Numerical Results}\label{Simulations}
We present some numerical results to illustrate the age performance of different policies. We consider different distributions for the packet service times with mean $1/\mu =1$, which are \emph{i.i.d.} across time and servers. The inter-generation times are \emph{i.i.d.} Erlang-2 distribution with mean $1/\lambda$. The number of servers is $m$. Hence, the traffic intensity is $\rho=\lambda/m\mu$\footnote{Throughout this section, the traffic intensity $\rho$ is computed as if there is no replication (i.e., $\rho$ is calculated when $r=1$).}. The queue size is $B$, which is a non-negative integer. 


%We consider the following reference policies for comparison: The FCFS policy with infinite buffer and buffer size B=1 was introduced in , 
 
\begin{figure}[t]
\centering
\includegraphics[scale=0.5]{figure/avg_age_m_1.eps}
\caption{Average age versus traffic intensity $\rho$ for an update system with $m=1$ server, queue size $B$, and exponential service times.}
%\vspace{-.1in}
\label{avg_age1}
\end{figure}
Figure \ref{avg_age1} illustrates the time-average age versus $\rho$ for an information-update system with $m=1$ server. The packet service times are exponentially distributed with mean 1. The time difference between packet generation and arrival ($a_i-s_i$) is zero, i.e., the update packets arrive in the same order of their generation times. We can observe that the prmp-LGFS-R policy achieves a better (smaller) age than the FCFS policy  analyzed in \cite{KaulYatesGruteser-Infocom2012}, and the non-preemptive LCFS policy with queue size $B=1$ \cite{2012CISS-KaulYatesGruteser} which was also named ``M/M/1/2*'' in \cite{CostaCodreanuEphremides2014ISIT}. 
Note that  in these prior studies, the time-average age was  characterized only for the special case of Poisson arrival process. Moreover, with ordered arrived packets at the server, the LGFS policy and LCFS policy have the same age performance.

%To validate the generality of our theoretical results, the arrival process considered here is different from the Poisson arrival process analyzed in \cite{KaulYatesGruteser-Infocom2012,2012ISIT-YatesKaul,2015ISITHuangModiano,CostaCodreanuEphremides2014ISIT}: 
%compared to the policies proposed in prior studies. 

Figure \ref{avg_peak_age2} plots the average peak age versus $\rho$ for an information-update system with $m=4$ servers. The packet service times are exponentially distributed with mean 1. The time difference between packet generation and arrival, i.e., $a_i-s_i$, is modeled to be either 1 or 100, with equal probability. The maximum replication degree $r$ is either 1, 2, or 4. For each $r$, we found that the prmp-LGFS-R policy achieves better age performance than all plotted policies that belong to the policy space $\Pi_r$ (e.g., the age performance of the prmp-LGFS-R policy when $r=2$ is better than the age performance of all policies that are plotted when $r$ equal to 1 and 2). It is important to emphasize that the age performance of the prmp-LGFS-R policy remains the same for any queue size $B\geq0$. However, the age performance of the non-prmp-LGFS-R policy and FCFS policy varies with the queue size $B$. We also observe that the average peak age in case of FCFS policy with $B=\infty$ blows up when the traffic intensity is high. This is due to the increased congestion in the network which leads to a delivery of stale packets. Moreover, in case of FCFS policy with $B=10$, the average peak age is high but bounded at high traffic intensity, since the fresh packet has a better opportunity to be delivered in a relatively short period compared with FCFS policy with $B=\infty$. These numerical result agrees with Theorem \ref{thm1}.

%the age performance of each policy is better than that in Fig. \ref{avg_age1}, because of the diversity provided by five servers.

%The plotted policies are FCFS policy with infinite buffer as introduced in \cite{KaulYatesGruteser-Infocom2012}, FCFS policy and non-preemptive LCFS policy with $B=1$ as introduced in \cite{CostaCodreanuEphremides2014ISIT,2012CISS-KaulYatesGruteser}, and preemptive LCFS policy \cite{2012CISS-KaulYatesGruteser}. We observe that, it is age optimal among all plotted policies for single server system. 

\begin{figure}[t]
\centering
\includegraphics[scale=0.5]{figure/Avg_peak_m_4_R124.eps}
\caption{Average peak age versus traffic intensity $\rho$ for an update system with $m=4$ servers, queue size $B$, maximum replication degree $r$, and exponential service times.}
%\vspace{-.2in}
\label{avg_peak_age2}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=0.5]{figure/Gamma_k_var_m4_ro_1dot8.eps}
\caption{Average age when the service times are gamma distributed versus the shape parameter $K$ for an update system with $m=4$ servers, queue size $B$, and maximum replication degree $r$.}
%\vspace{-.2in}
\label{avg_peak_age3}
\end{figure}

Figure \ref{avg_peak_age3} plots the average age when the service times are gamma distributed versus the shape parameter $K$ for an information-update system with $m=4$ servers and $\rho=1.8$. The mean of the gamma service time distribution is 1. The time difference between packet generation and arrival ($a_i-s_i$) is zero. The maximum replication degree $r$ is either 1 or 4. \textcolor[rgb]{0.00,0.00,1.00}{The "Age lower bound'' curve is generated by using $\frac{\int_0^{T} \phi_{\text{LB}}(t)dt}{T}$ when $B=1$ and $r=1$ which, according to Lemma \ref{lowerbound_lemma}, is a lower bound of the optimum average age. We can observe that the gap between the "Age lower bound'' curve and the average age of the non-prmp-LGFS-R policy when $r=1$ does not exceed 1 (the mean service time), which agrees with Theorem \ref{thmNBU1}.} In addition, we can notice that packet replication can improve the age performance. In particular, we found that the non-prmp-LGFS-R policy when $r=4$ has the best age performance among all plotted causal policies when the shape parameter $K$ is between 2 and 6.5. This is a surprising result since it was shown in \cite{sun2016delay} that replication policies are far from the optimum delay and throughput for NBU service time distributions.  Furthermore, we can observe that the average age of the non-prmp-LGFS-R policy increases as the shape parameter $K$ increases. An explanation of this observation is that as the shape parameter $K$ increases, the variance (variability) of the gamma service time decreases until it becomes close to be constant. This, in turn, reduces the benefit gained from the diversity provided by four servers and hence increases the average age. Finally, we can observe that prmp-LGFS-R policy achieves the best age performance among all plotted causal policies when $K=1$. This is because a gamma distribution with shape parameter $K=1$ is an exponential distribution. Thus, age-optimality can be achieved in this case by policy prmp-LGFS-R as stated in Theorem \ref{thm1}. However, as can be seen in the figure, the average age of the prmp-LGFS-R policy blows up as the shape parameter $K$ increases. This is because the packet service times are no longer memoryless. Moreover, as $K$ increases, the variance (variability) of the gamma service time decreases (i.e., the gamma distribution is close to be constant at high $K$). Thus, high traffic intensity leads to increased preemption rate which, in turn, leads to large inter-departure times and hence high age. This agrees with the claim mentioned in the conclusion of \cite[Appendix]{CostaCodreanuEphremides_TIT}. 
 





























%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.5]{figure/Avg_peak_m_5_R.eps}
%\caption{Average peak age versus traffic intensity $\rho$ for an update system with $m=5$ servers and queue size $B$.}
%%\vspace{-.2in}
%\label{avg_peak_age3}
%\end{figure}
%
%Figure \ref{avg_peak_age3} plots  the Average peak age versus $\rho$ for an information-update system with $m=5$ servers. The packet service times are exponentially distributed. The plotted policies are the same as those in Fig. \ref{avg_age1} beside the non-prmp-LGFS-R and prmp-LGFS-R policies. We found that packet replication improves the age performance dramatically. In addition, the prmp-LGFS-R policy achieves the best age performance among all plotted policies. These numerical result shows agreement with Theorem \ref{thm1R}.
%
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.5]{figure/deterministic-Gap.eps}
%\caption{Average age versus traffic intensity $\rho$ for an update system with $m=5$ servers and queue size $B$.}
%%\vspace{-.2in}
%\label{avg_age4}
%\end{figure}
%Figure \ref{avg_age4} illustrates the time-average age versus $\rho$ for an information-update system with $m=5$ server. The packet service times are constant with value 1. The time difference between packet generation and arrival ($a_i-s_i$) is zero, i.e., the update packets arrive in the same order of their generation times. The plotted policies are the prmp-LGFS policy, non-prmp-LGFS policy and the lower bound constructed in Appendix~\ref{Appendix_D}. As can be seen in the figure, the gap between the lower bound and the average age of non-prmp-LGFS policy is exactly one which is the value of the service time. We also notice the the prmp-LGFS policy is no longer an age-optimal. In particular,  the average age of the prmp-LGFS policy blows up when the traffic intensity is high. This is because the packet service times are no longer memoryless. Thus, high traffic intensity leads to increased preemption rate which for its part leads to large inter-departure times and hence high age.
%
%
%
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.5]{figure/gama_k_2_theta_half_mean_1.eps}
%\caption{Average age versus traffic intensity $\rho$ for an update system with $m=5$ servers and queue size $B$.}
%%\vspace{-.2in}
%\label{avg_age5}
%\end{figure}
%
%Figure \ref{avg_age5} illustrates the time-average age versus $\rho$ for an information-update system with $m=5$ server. The packet service times are gamma distributed with shape parameter $k=2$. The time difference between packet generation and arrival ($a_i-s_i$) is zero. The plotted policies are the non-prmp-LGFS policy and non-prmp-LGFS-R policy. We can observe that the non-prmp-LGFS-R policy has a lower time-average age than that of non-prmp-LGFS policy, i.e., packet replication improves the age performance of non-prmp-LGFS policy. However, it is obvious that when the packet service times are constant, packet replication is no longer helpful because the replicated packets spend the same time at all servers. From this we can conclude that, packet replication affects the age performance of the scheduling policies depending on the service time distributions. 

